An extended physics informed neural network for preliminary analysis of parametric optimal control problems

In this work we propose an extension of physics informed supervised learning strategies to parametric partial differential equations. Indeed, even if the latter are indisputably useful in many applications, they can be computationally expensive most of all in a real-time and many-query setting. Thus, our main goal is to provide a physics informed learning paradigm to simulate parametrized phenomena in a small amount of time. The physics information will be exploited in many ways, in the loss function (standard physics informed neural networks), as an augmented input (extra feature employment) and as a guideline to build an effective structure for the neural network (physics informed architecture). These three aspects, combined together, will lead to a faster training phase and to a more accurate parametric prediction. The methodology has been tested for several equations and also in an optimal control framework.

==> sections/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{tikz}
\usepackage{tikzsymbols}
\usepackage{comment}
\usepackage{mathrsfs}
\usepackage{float}
\usepackage[scientific-notation=true]{siunitx}


\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,%
    decorations.pathreplacing,decorations.pathmorphing,shapes,%
    matrix,shapes.symbols, decorations.markings, patterns,fit,quotes,%
    arrows.meta}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}


\newcommand{\TODO}[1]{{\color{red}#1}}
\newcommand{\Maria}[1]{{\color{teal}#1}}
\newcommand{\ND}[1]{{\color{purple}#1}}

\newcommand{\mupar}{\ensuremath{\boldsymbol{\mu}}}
\newcommand{\etapar}{\ensuremath{\boldsymbol{\eta}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\fulldim}{\ensuremath{\mathcal{N}}}
\newcommand{\reddim}{\ensuremath{N}}
\newcommand{\pardim}{\ensuremath{m}}
\newcommand{\norm}[1]{\lVert #1 \rVert}

\newcommand{\A}[1]{\color{blue}{ #1}\color{black}}



% Used for creating new theorem and remark environments
%\newsiamremark{remark}{Remark}
%\newsiamremark{hypothesis}{Hypothesis}
%\crefname{hypothesis}{Hypothesis}{Hypotheses}
%\newsiamthm{claim}{Claim}
\newdefinition{remark}{Remark}

% Sets running headers as well as PDF title and authors
%\headers{Extended PINNs: a first application to OCP($\mupar$)s}{N. Demo, M. Strazzullo, and G. Rozza}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
%\title{%
%An extended physics informed neural network for preliminary analysis of parametric optimal control problems}

% Authors: full names plus addresses.
%\author{Nicola~Demo\thanks{SISSA, Mathematics Area, mathLab, via Bonomea 265, I-34136
%  Trieste, Italy 
%  (\email{nicola.demo@sissa.it}, \email{maria.strazzullo@sissa.it}, \email{gianluigi.rozza@sissa.it})}.
%\and Maria~Strazzullo$^{*}$
%\and Gianluigi~Rozza$^{*}$}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> sections/preamble.tex <==
%\usepackage{subfig}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

\usepackage{amsmath}
\usepackage{multirow}
%\usepackage[table]{xcolor}
\usepackage{subcaption}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{fillbetween}
\usepackage{mathtools}
\usepackage{multicol}
\usepackage{comment}
\usepackage{booktabs}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{mathrsfs}
\usepackageion=true]{siunitx}
%\usepackage[doublespacing]{setspace}

%\usepackage{pdfsync}

\usepackage{float}
%\usepackage{tabularx}
\usepackage{enumerate}
\usepackage{array}
\usepackage{xspace}
\usepackage{tikz}
\usepackage{tikzsymbols}
\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,%
    decorations.pathreplacing,decorations.pathmorphing,shapes,%
    matrix,shapes.symbols, decorations.markings, patterns,fit,quotes,%
    arrows.meta}

\usepackage{authblk}
%\usepackage{xcolor}
%\definecolor{Gray}{gray}{0.9}

%\usepackage{hyperref}
%\usepackage{siunitx}
%\UseRawInputEncoding
%\usepackage[bottom]{footmisc}
%\usepackage[draft,inline,marginclue]{fixme}
% add yours
%\FXRegisterAuthor{mt}{amt}{MT}
%\newcommand{\MT}[1]{\mtwarning{#1}}

%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{corol}{Corollary}
%\newtheorem{remark}{Remark}


\newcommand{\TODO}[1]{{\color{red}#1}}
\newcommand{\Maria}[1]{{\color{teal}#1}}
\newcommand{\ND}[1]{{\color{purple}#1}}

\newcommand{\mupar}{\ensuremath{\boldsymbol{\mu}}}
\newcommand{\etapar}{\ensuremath{\boldsymbol{\eta}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\fulldim}{\ensuremath{\mathcal{N}}}
\newcommand{\reddim}{\ensuremath{N}}
\newcommand{\pardim}{\ensuremath{m}}
\newcommand{\norm}[1]{\lVert #1 \rVert}

\newcommand{\fullspace}{\ensuremath{\mathbb{X}^\fulldim}}
\newcommand{\redspace}{\ensuremath{\mathbb{X}^\fulldim_\reddim}}
\newcommand{\parspace}{\ensuremath{{\bf P}}}
%\newcommand{\Xtrain}{\ensuremath{\mathbf{X}}}
%\newcommand{\Xtest}{\ensuremath{\mathbf{\Bar{X}}}}
%\newcommand{\ytrain}{\ensuremath{\mathbf{y}}}
%\newcommand{\ytest}{\ensuremath{\mathbf{\Bar{y}}}}


%\newcommand{\RA}[1]{{\color{black}#1}}
%\newcommand{\RB}[1]{{\color{black}#1}}
%\newcommand{\RC}[1]{{\color{black}#1}}

\headers{Extended PINNs for OCP($\mupar$)s}{N. Demo, M. Strazzullo, and G. Rozza}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{%
An extended physics informed neural network for preliminary analysis of parametric optimal control problems}

% Authors: full names plus addresses.
\author{Nicola~Demo\thanks{SISSA, Mathematics Area, mathLab, via Bonomea 265, I-34136
  Trieste, Italy 
  (\email{nicola.demo@sissa.it}).}
\and Maria~Strazzullo\thanks{SISSA, Mathematics Area, mathLab, via Bonomea 265, I-34136
  Trieste, Italy (\email{maria.strazzullo@sissa.it}).}
\and Gianluigi~Rozza\thanks{SISSA, Mathematics Area, mathLab, via Bonomea 265, I-34136
  Trieste, Italy (\email{gianluigi.rozza@sissa.it}).}}


